ProVe: A Pipeline for Automated Provenance Verification of Knowledge Graphs against Textual Sources

Knowledge Graphs are repositories of information that gather data from a multitude of domains and sources in the form of semantic triples, serving as a source of structured data for various crucial applications in the modern web landscape, from Wikipedia infoboxes to search engines. Such graphs mainly serve as secondary sources of information and depend on well-documented and verifiable provenance to ensure their trustworthiness and usability. However, their ability to systematically assess and assure the quality of this provenance, most crucially whether it properly supports the graph's information, relies mainly on manual processes that do not scale with size. ProVe aims at remedying this, consisting of a pipelined approach that automatically verifies whether a Knowledge Graph triple is supported by text extracted from its documented provenance. ProVe is intended to assist information curators and consists of four main steps involving rule-based methods and machine learning models: text extraction, triple verbalisation, sentence selection, and claim verification. ProVe is evaluated on a Wikidata dataset, achieving promising results overall and excellent performance on the binary classification task of detecting support from provenance, with 87.5% accuracy and 82.9% F1-macro on text-rich sources. The evaluation data and scripts used in this paper are available on GitHub and Figshare.

==> sections/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conc} % 0.5 page

%You: Do we need to talk here on future work, or is it enough what we covered in %discussion/limitations?
%
%Elena Simperl: You should cover it, but you could equally merge this section with the %discussion one, call it, discussion and conclusions because it does repeat a lot of the %stuff from earlier.

Wikidata, such as any other collaborative knowledge base, has an huge potential as a secondary source of information. Ensuring the verifiability of its data through references is a task that is crucial to its editorial process and should be actively supported by automated and semi-automated tools to help editors cope with the sheer volume of information. However, as of now, there are none deployed and a very small family of approaches that fit such specific formulation.

In this paper, we propose, develop, and evaluate such a tool. POSE leverages large pre-trained LMs, rule-based methods, and simple classifiers, to provide automated assistance to the activity of creating and maintaining references in a KG, with a use-case centered around Wikidata. POSE's pipeline aims at extracting relevant textual information from references and judges whether or not they they support a given KG claim, providing editors with a final classification, as well as relevance and textual entailment metrics for each retrieved sentence. Such a tool, deployed correctly, can help editors detect potential verifiability issues in existing references, as well as improve the reuse of good sources. Additionally, the approach can be feasibly expanded to work in a multilingual setting.

We evaluate POSE with WTR, a dataset of claim-reference pairs extracted directly from Wikidata and annotated by both crowdworkers and the authors. POSE achieves $75\%$ accuracy, $0.681$ F1-macro, and $0.667$ AUC on the full evaluation dataset, which include web pages from many different domains. On references where support is stated explicitly and in natural text, POSE achieves an excellent 87.5\% accurac (0.829 F1-macro and 0.908 AUC).

Additionally, WTR can be used as a benchmarking dataset for future approaches to KG claim verification on textual references from multiple types of web domains, not only Wikipedia. Our crowdsourcing tasks, whose code and implementation is available on GitHub, can also be reused for similar studies.

\subsubsection*{Acknowledgements} This research received funding from the European Union’s Horizon 2020 research and innovation programme under the Marie Skłodowska-Curie grant agreement no. 812997.
